FreeGuard: A Faster Secure Heap Allocator

In spite of years of improvements to software security, heap-related attacks still remain a severe threat. One reason is that many existing memory allocators fall short in a variety of aspects. For instance, performance-oriented allocators are designed with very limited countermeasures against attacks, but secure allocators generally suffer from significant performance overhead, e.g., running up to 10x slower. This paper, therefore, introduces FreeGuard, a secure memory allocator that prevents or reduces a wide range of heap-related attacks, such as heap overflows, heap over-reads, use-after-frees, as well as double and invalid frees. FreeGuard has similar performance to the default Linux allocator, with less than 2% overhead on average, but provides significant improvement to security guarantees. FreeGuard also addresses multiple implementation issues of existing secure allocators, such as the issue of scalability. Experimental results demonstrate that FreeGuard is very effective in defending against a variety of heap-related attacks.

==> glyphtounicode.tex <==
%
% Copyright (c) 2008,  Han The Thanh <thanh@river-valley.org>
% Copyright (c) 2014,  Peter Selinger <selinger@mathstat.dal.ca>
%                      
%  This file may be distributed and/or modified under the conditions
%  of the LaTeX Project Public License, either version 1.2 of this
%  license or (at your option) any later version.  The latest version
%  of this license is in:
%    
%    http://www.latex-project.org/lppl.txt
%    
%  and version 1.2 or later is part of all distributions of LaTeX
%  version 1999/12/01 or later.
%
% Changes:
% 2014/08/11: PS1 - mapped most glyphs to existing Unicode code points.
% 2014/08/11: PS1 - added mappings for the xyatip and xybtip fonts.

%% Glyphs from the cmex fonts:

\pdfglyphtounicode{angbracketleftBig}{27E8}
\pdfglyphtounicode{angbracketleftBigg}{27E8}
\pdfglyphtounicode{angbracketleftbig}{27E8}
\pdfglyphtounicode{angbracketleftbigg}{27E8}
\pdfglyphtounicode{angbracketrightBig}{27E9}
\pdfglyphtounicode{angbracketrightBigg}{27E9}
\pdfglyphtounicode{angbracketrightbig}{27E9}
\pdfglyphtounicode{angbracketrightbigg}{27E9}
\pdfglyphtounicode{arrowbt}{2193}
\pdfglyphtounicode{arrowdblbt}{21D3}
\pdfglyphtounicode{arrowdbltp}{21D1}
\pdfglyphtounicode{arrowhookleft}{21AA}
\pdfglyphtounicode{arrowhookright}{21A9}
\pdfglyphtounicode{arrowtp}{2191}
\pdfglyphtounicode{arrowvertex}{23D0}
\pdfglyphtounicode{arrowvertexdbl}{ED12}
\pdfglyphtounicode{backslashBig}{005C}
\pdfglyphtounicode{backslashBigg}{005C}
\pdfglyphtounicode{backslashbig}{005C}
\pdfglyphtounicode{backslashbigg}{005C}
\pdfglyphtounicode{braceex}{23AA}
\pdfglyphtounicode{bracehtipdownleft}{ED17}
\pdfglyphtounicode{bracehtipdownright}{ED18}
\pdfglyphtounicode{bracehtipupleft}{ED19}
\pdfglyphtounicode{bracehtipupright}{ED1A}
\pdfglyphtounicode{braceleftBig}{007B}
\pdfglyphtounicode{braceleftBigg}{007B}
\pdfglyphtounicode{braceleftbig}{007B}
\pdfglyphtounicode{braceleftbigg}{007B}
\pdfglyphtounicode{braceleftbt}{23A9}
\pdfglyphtounicode{braceleftmid}{23A8}
\pdfglyphtounicode{bracelefttp}{23A7}
\pdfglyphtounicode{bracerightBig}{007D}
\pdfglyphtounicode{bracerightBigg}{007D}
\pdfglyphtounicode{bracerightbig}{007D}
\pdfglyphtounicode{bracerightbigg}{007D}
\pdfglyphtounicode{bracerightbt}{23AD}
\pdfglyphtounicode{bracerightmid}{23AC}
\pdfglyphtounicode{bracerighttp}{23AB}
\pdfglyphtounicode{bracketleftBig}{005B}
\pdfglyphtounicode{bracketleftBigg}{005B}
\pdfglyphtounicode{bracketleftbig}{005B}
\pdfglyphtounicode{bracketleftbigg}{005B}
\pdfglyphtounicode{bracketleftbt}{23A3}
\pdfglyphtounicode{bracketleftex}{23A2}
\pdfglyphtounicode{bracketlefttp}{23A1}
\pdfglyphtounicode{bracketrightBig}{005D}
\pdfglyphtounicode{bracketrightBigg}{005D}
\pdfglyphtounicode{bracketrightbig}{005D}
\pdfglyphtounicode{bracketrightbigg}{005D}
\pdfglyphtounicode{bracketrightbt}{23A6}
\pdfglyphtounicode{bracketrightex}{23A5}
\pdfglyphtounicode{bracketrighttp}{23A4}
\pdfglyphtounicode{ceilingleftBig}{2308}
\pdfglyphtounicode{ceilingleftBigg}{2308}
\pdfglyphtounicode{ceilingleftbig}{2308}
\pdfglyphtounicode{ceilingleftbigg}{2308}
\pdfglyphtounicode{ceilingrightBig}{2309}
\pdfglyphtounicode{ceilingrightBigg}{2309}
\pdfglyphtounicode{ceilingrightbig}{2309}
\pdfglyphtounicode{ceilingrightbigg}{2309}
\pdfglyphtounicode{circledotdisplay}{2A00}
\pdfglyphtounicode{circledottext}{2A00}
\pdfglyphtounicode{circlemultiplydisplay}{2A02}
\pdfglyphtounicode{circlemultiplytext}{2A02}
\pdfglyphtounicode{circleplusdisplay}{2A01}
\pdfglyphtounicode{circleplustext}{2A01}
\pdfglyphtounicode{contintegraldisplay}{222E}
\pdfglyphtounicode{contintegraltext}{222E}
\pdfglyphtounicode{coproductdisplay}{2210}
\pdfglyphtounicode{coproducttext}{2210}
\pdfglyphtounicode{floorleftBig}{230A}
\pdfglyphtounicode{floorleftBigg}{230A}
\pdfglyphtounicode{floorleftbig}{230A}
\pdfglyphtounicode{floorleftbigg}{230A}
\pdfglyphtounicode{floorrightBig}{230B}
\pdfglyphtounicode{floorrightBigg}{230B}
\pdfglyphtounicode{floorrightbig}{230B}
\pdfglyphtounicode{floorrightbigg}{230B}
\pdfglyphtounicode{hatwide}{02C6}
\pdfglyphtounicode{hatwider}{02C6}
\pdfglyphtounicode{hatwidest}{02C6}
\pdfglyphtounicode{integraldisplay}{222B}
\pdfglyphtounicode{integraltext}{222B}
\pdfglyphtounicode{intersectiondisplay}{22C2}
\pdfglyphtounicode{intersectiontext}{22C2}
\pdfglyphtounicode{logicalanddisplay}{22C0}
\pdfglyphtounicode{logicalandtext}{22C0}
\pdfglyphtounicode{logicalordisplay}{22C1}
\pdfglyphtounicode{logicalortext}{22C1}
\pdfglyphtounicode{mapsto}{21A6}
\pdfglyphtounicode{parenleftBig}{0028}
\pdfglyphtounicode{parenleftBigg}{0028}
\pdfglyphtounicode{parenleftbig}{0028}
\pdfglyphtounicode{parenleftbigg}{0028}
\pdfglyphtounicode{parenleftbt}{239D}
\pdfglyphtounicode{parenleftex}{239C}
\pdfglyphtounicode{parenlefttp}{239B}
\pdfglyphtounicode{parenrightBig}{0029}
\pdfglyphtounicode{parenrightBigg}{0029}
\pdfglyphtounicode{parenrightbig}{0029}
\pdfglyphtounicode{parenrightbigg}{0029}
\pdfglyphtounicode{parenrightbt}{23A0}
\pdfglyphtounicode{parenrightex}{239F}
\pdfglyphtounicode{parenrighttp}{239E}
\pdfglyphtounicode{productdisplay}{220F}
\pdfglyphtounicode{producttext}{220F}
\pdfglyphtounicode{radicalBig}{221A}
\pdfglyphtounicode{radicalBigg}{221A}
\pdfglyphtounicode{radicalbig}{221A}
\pdfglyphtounicode{radicalbigg}{221A}
\pdfglyphtounicode{radicalbt}{221A}
\pdfglyphtounicode{radicaltp}{ED6A}
\pdfglyphtounicode{radicalvertex}{ED6B}
\pdfglyphtounicode{slashBig}{002F}
\pdfglyphtounicode{slashBigg}{002F}
\pdfglyphtounicode{slashbig}{002F}
\pdfglyphtounicode{slashbigg}{002F}
\pdfglyphtounicode{summationdisplay}{2211}
\pdfglyphtounicode{summationtext}{2211}
\pdfglyphtounicode{tie}{2040}
\pdfglyphtounicode{tildewide}{02DC}
\pdfglyphtounicode{tildewider}{02DC}
\pdfglyphtounicode{tildewidest}{02DC}
\pdfglyphtounicode{uniondisplay}{22C3}
\pdfglyphtounicode{unionmultidisplay}{2A04}
\pdfglyphtounicode{unionmultitext}{2A04}
\pdfglyphtounicode{unionsqdisplay}{2A06}
\pdfglyphtounicode{unionsqtext}{2A06}
\pdfglyphtounicode{uniontext}{22C3}
\pdfglyphtounicode{vextenddouble}{ED79}
\pdfglyphtounicode{vextendsingle}{23D0}

%% Glyphs from the cmr fonts:

\pdfglyphtounicode{suppress}{EB61}

%% Glyphs from the lasy fonts:

%% Note: unfortunately, some other fonts, such as line and xydash,
%% also use glyphs names a0...a127, but for different glyphs.

\pdfglyphtounicode{a1}{25C1}
\pdfglyphtounicode{a2}{22B4}
\pdfglyphtounicode{a3}{25B7}
\pdfglyphtounicode{a4}{22B5}
\pdfglyphtounicode{a40}{02C2}
\pdfglyphtounicode{a41}{02C3}
\pdfglyphtounicode{a42}{2303}
\pdfglyphtounicode{a43}{2304}
\pdfglyphtounicode{a48}{2127}
\pdfglyphtounicode{a49}{22C8}
\pdfglyphtounicode{a50}{25A1}
\pdfglyphtounicode{a51}{25C7}
\pdfglyphtounicode{a58}{2053}
\pdfglyphtounicode{a59}{219D}
\pdfglyphtounicode{a60}{228F}
\pdfglyphtounicode{a61}{2290}

%% Glyphs from the xyatip and xybtip fonts fonts of the XYPic package.
%% They denote half arrow tips pointing in various directions.  We map
%% them to Unicode arrows pointing in approximately the same
%% direction, in increments of 45 degrees.

\pdfglyphtounicode{d0}{2199}
\pdfglyphtounicode{d1}{2199}
\pdfglyphtounicode{d2}{2199}
\pdfglyphtounicode{d3}{2199}
\pdfglyphtounicode{d4}{2199}
\pdfglyphtounicode{d5}{2199}
\pdfglyphtounicode{d6}{2199}
\pdfglyphtounicode{d7}{2193}
\pdfglyphtounicode{d8}{2193}
\pdfglyphtounicode{d9}{2193}
\pdfglyphtounicode{d10}{2193}
\pdfglyphtounicode{d11}{2193}
\pdfglyphtounicode{d12}{2193}
\pdfglyphtounicode{d13}{2193}
\pdfglyphtounicode{d14}{2193}
\pdfglyphtounicode{d15}{2193}
\pdfglyphtounicode{d16}{2193}
\pdfglyphtounicode{d17}{2193}
\pdfglyphtounicode{d18}{2193}
\pdfglyphtounicode{d19}{2193}
\pdfglyphtounicode{d20}{2193}
\pdfglyphtounicode{d21}{2193}
\pdfglyphtounicode{d22}{2193}
\pdfglyphtounicode{d23}{2193}
\pdfglyphtounicode{d24}{2198}
\pdfglyphtounicode{d25}{2198}
\pdfglyphtounicode{d26}{2198}
\pdfglyphtounicode{d27}{2198}
\pdfglyphtounicode{d28}{2198}
\pdfglyphtounicode{d29}{2198}
\pdfglyphtounicode{d30}{2198}
\pdfglyphtounicode{d31}{2198}
\pdfglyphtounicode{d32}{2198}
\pdfglyphtounicode{d33}{2198}
\pdfglyphtounicode{d34}{2198}
\pdfglyphtounicode{d35}{2198}
\pdfglyphtounicode{d36}{2198}
\pdfglyphtounicode{d37}{2198}
\pdfglyphtounicode{d38}{2198}
\pdfglyphtounicode{d39}{2192}
\pdfglyphtounicode{d40}{2192}
\pdfglyphtounicode{d41}{2192}
\pdfglyphtounicode{d42}{2192}
\pdfglyphtounicode{d43}{2192}
\pdfglyphtounicode{d44}{2192}
\pdfglyphtounicode{d45}{2192}
\pdfglyphtounicode{d46}{2192}
\pdfglyphtounicode{d47}{2192}
\pdfglyphtounicode{d48}{2192}
\pdfglyphtounicode{d49}{2192}
\pdfglyphtounicode{d50}{2192}
\pdfglyphtounicode{d51}{2192}
\pdfglyphtounicode{d52}{2192}
\pdfglyphtounicode{d53}{2192}
\pdfglyphtounicode{d54}{2192}
\pdfglyphtounicode{d55}{2192}
\pdfglyphtounicode{d56}{2197}
\pdfglyphtounicode{d57}{2197}
\pdfglyphtounicode{d58}{2197}
\pdfglyphtounicode{d59}{2197}
\pdfglyphtounicode{d60}{2197}
\pdfglyphtounicode{d61}{2197}
\pdfglyphtounicode{d62}{2197}
\pdfglyphtounicode{d63}{2197}
\pdfglyphtounicode{d64}{2197}
\pdfglyphtounicode{d65}{2197}
\pdfglyphtounicode{d66}{2197}
\pdfglyphtounicode{d67}{2197}
\pdfglyphtounicode{d68}{2197}
\pdfglyphtounicode{d69}{2197}
\pdfglyphtounicode{d70}{2197}
\pdfglyphtounicode{d71}{2191}
\pdfglyphtounicode{d72}{2191}
\pdfglyphtounicode{d73}{2191}
\pdfglyphtounicode{d74}{2191}
\pdfglyphtounicode{d75}{2191}
\pdfglyphtounicode{d76}{2191}
\pdfglyphtounicode{d77}{2191}
\pdfglyphtounicode{d78}{2191}
\pdfglyphtounicode{d79}{2191}
\pdfglyphtounicode{d80}{2191}
\pdfglyphtounicode{d81}{2191}
\pdfglyphtounicode{d82}{2191}
\pdfglyphtounicode{d83}{2191}
\pdfglyphtounicode{d84}{2191}
\pdfglyphtounicode{d85}{2191}
\pdfglyphtounicode{d86}{2191}
\pdfglyphtounicode{d87}{2191}
\pdfglyphtounicode{d88}{2196}
\pdfglyphtounicode{d89}{2196}
\pdfglyphtounicode{d90}{2196}
\pdfglyphtounicode{d91}{2196}
\pdfglyphtounicode{d92}{2196}
\pdfglyphtounicode{d93}{2196}
\pdfglyphtounicode{d94}{2196}
\pdfglyphtounicode{d95}{2196}
\pdfglyphtounicode{d96}{2196}
\pdfglyphtounicode{d97}{2196}
\pdfglyphtounicode{d98}{2196}
\pdfglyphtounicode{d99}{2196}
\pdfglyphtounicode{d100}{2196}
\pdfglyphtounicode{d101}{2196}
\pdfglyphtounicode{d102}{2196}
\pdfglyphtounicode{d103}{2190}
\pdfglyphtounicode{d104}{2190}
\pdfglyphtounicode{d105}{2190}
\pdfglyphtounicode{d106}{2190}
\pdfglyphtounicode{d107}{2190}
\pdfglyphtounicode{d108}{2190}
\pdfglyphtounicode{d109}{2190}
\pdfglyphtounicode{d110}{2190}
\pdfglyphtounicode{d111}{2190}
\pdfglyphtounicode{d112}{2190}
\pdfglyphtounicode{d113}{2190}
\pdfglyphtounicode{d114}{2190}
\pdfglyphtounicode{d115}{2190}
\pdfglyphtounicode{d116}{2190}
\pdfglyphtounicode{d117}{2190}
\pdfglyphtounicode{d118}{2190}
\pdfglyphtounicode{d119}{2190}
\pdfglyphtounicode{d120}{2199}
\pdfglyphtounicode{d121}{2199}
\pdfglyphtounicode{d122}{2199}
\pdfglyphtounicode{d123}{2199}
\pdfglyphtounicode{d124}{2199}
\pdfglyphtounicode{d125}{2199}
\pdfglyphtounicode{d126}{2199}
\pdfglyphtounicode{d127}{2199}
\endinput

% Reference:
%
% http://codepoints.net/basic_latin
% 0028 0029 002F 005B 005C 005D 007B 007D
%
% http://codepoints.net/spacing_modifier_letters
% 02C2 02C3 02C6 02DC
%
% http://codepoints.net/general_punctuation
% 2040 2053
%
% http://codepoints.net/letterlike_symbols
% 2127
%
% http://codepoints.net/arrows
% 2190 2191 2192 2193 2196 2197 2198 2199 219D 21A6 21A9 21AA 21D1 21D3
%
% http://codepoints.net/mathematical_operators
% 220F 2210 2211 221A 222B 222E 228F 2290 22B4 22B5 22C0 22C1 22C2 22C3
% 22C8
%
% http://codepoints.net/miscellaneous_technical
% 2303 2304 2308 2309 230A 230B 239B 239C 239D 239E 239F 23A0 23A1 23A2
% 23A3 23A4 23A5 23A6 23A7 23A8 23A9 23AA 23AB 23AC 23AD 23D0
%
% http://codepoints.net/geometric_shapes
% 25A1 25B7 25C1 25C7
%
% http://codepoints.net/miscellaneous_mathematical_symbols-a
% 27E8 27E9
%
% http://codepoints.net/supplemental_mathematical_operators
% 2A00 2A01 2A02 2A04 2A06
%
% Private Use Area:
% EB61 ED12 ED17 ED18 ED19 ED1A ED6A ED6B ED79

%
%
% End of file 'glyphtounicode-cmr.tex
%


